LoCuSS: First Results from Strong-lensing Analysis of 20 Massive Galaxy Clusters at z~0.2

We present a statistical analysis of a sample of 20 strong lensing clusters drawn from the Local Cluster Substructure Survey (LoCuSS), based on high resolution Hubble Space Telescope imaging of the cluster cores and follow-up spectroscopic observations using the Keck-I telescope. We use detailed parameterized models of the mass distribution in the cluster cores, to measure the total cluster mass and fraction of that mass associated with substructures within R<250kpc.These measurements are compared with the distribution of baryons in the cores, as traced by the old stellar populations and the X-ray emitting intracluster medium. Our main results include: (i) the distribution of Einstein radii is log-normal, with a peak and 1sigma width of <log(RE(z=2))>=1.16+/-0.28; (ii) we detect an X-ray/lensing mass discrepancy of <M_SL/M_X>=1.3 at 3 sigma significance -- clusters with larger substructure fractions displaying greater mass discrepancies, and thus greater departures from hydrostatic equilibrium; (iii) cluster substructure fraction is also correlated with the slope of the gas density profile on small scales, implying a connection between cluster-cluster mergers and gas cooling. Overall our results are consistent with the view that cluster-cluster mergers play a prominent role in shaping the properties of cluster cores, in particular causing departures from hydrostatic equilibrium, and possibly disturbing cool cores. Our results do not support recent claims that large Einstein radius clusters present a challenge to the CDM paradigm.

==> spectra/dospec <==
#!/usr/local/bin/perl

open(IN,$ARGV[0])||die;

print "\\begin{figure*}\n";
print "\\caption{\\label{spectra}Extracted spectra of multiple images from the current sample. We mark the proeminent spectral 
features used to derive the redshift.}\n";

$i=0;
while(<IN>)
{
   @Fld=split;
   print "\\begin{minipage}{5.5cm}\n";
   print "\\centerline{$Fld[2]}\n";
   print "\\includegraphics[height=4.5cm,angle=270]{spectra/$Fld[2]_1d.ps}\n";
   print "\\end{minipage}\n";
   $i++;
   if($i==15)
   {
     $i=0;
     print "\\end{figure*}\n";
     print "\\begin{figure*}\n";
   }
}
print "\\end{figure*}\n";


==> spectra/spec.tex <==
\begin{figure*}
\caption{\label{spectra}Extracted spectra of multiple images from the current sample. We mark the proeminent spectral 
features used to derive the redshift.}
\begin{minipage}{7cm}
\centerline{A521-1.1}
\includegraphics[height=6.0cm,angle=270]{spectra/A521-1.1_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A521-1.2}
\includegraphics[height=6.0cm,angle=270]{spectra/A521-1.2_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A521-1.3}
\includegraphics[height=6.0cm,angle=270]{spectra/A521-1.3_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A611-1.2+1.3}
\includegraphics[height=6.0cm,angle=270]{spectra/A611-1.2+1.3_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A611-2.1+2.2}
\includegraphics[height=6.0cm,angle=270]{spectra/A611-2.1+2.2_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A611-2.3}
\includegraphics[height=6.0cm,angle=270]{spectra/A611-2.3_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A611-4.1}
\includegraphics[height=6.0cm,angle=270]{spectra/A611-4.1_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A773-1.1}
\includegraphics[height=6.0cm,angle=270]{spectra/A773-1.1_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A773-1.2}
\includegraphics[height=6.0cm,angle=270]{spectra/A773-1.2_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A773-2.1}
\includegraphics[height=6.0cm,angle=270]{spectra/A773-2.1_1d.ps}
\end{minipage}
\end{figure*}
\begin{figure*}
\begin{minipage}{7cm}
\centerline{A773-3.1}
\includegraphics[height=6.0cm,angle=270]{spectra/A773-3.1_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A868-1.1+1.2}
\includegraphics[height=6.0cm,angle=270]{spectra/A868-1.1+1.2_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{Z2701-1.1}
\includegraphics[height=6.0cm,angle=270]{spectra/Z2701-1.1_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{Z2701-1.3}
\includegraphics[height=6.0cm,angle=270]{spectra/Z2701-1.3_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A1413-1.1+1.2}
\includegraphics[height=6.0cm,angle=270]{spectra/A1413-1.1+1.2_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A1413-2.1+2.2}
\includegraphics[height=6.0cm,angle=270]{spectra/A1413-2.1+2.2_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A1413-3.1+3.2+3.3}
\includegraphics[height=6.0cm,angle=270]{spectra/A1413-3.1+3.2+3.3_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A1835-7.1}
\includegraphics[height=6.0cm,angle=270]{spectra/A1835-7.1_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A2204-1.1}
\includegraphics[height=6.0cm,angle=270]{spectra/A2204-1.1_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{A2204-1.2}
\includegraphics[height=6.0cm,angle=270]{spectra/A2204-1.2_1d.ps}
\end{minipage}
\end{figure*}
\begin{figure*}
\begin{minipage}{7cm}
\centerline{RXJ1720-1.1+1.2}
\includegraphics[height=6.0cm,angle=270]{spectra/RXJ1720-1.1+1.2_1d.ps}
\end{minipage}
\begin{minipage}{7cm}
\centerline{RXJ2129-1.1}
\includegraphics[height=6.0cm,angle=270]{spectra/RXJ2129-1.1_1d.ps}
\end{minipage}
\end{figure*}


==> spectra/spec1d <==
#!/usr/bin/perl

use PGPLOT;

open(IN,$ARGV[0])||die;
while(<IN>)
{
    @Fld=split;

    $id2=$Fld[0];
    $z=$Fld[1];
    $id=$Fld[2];
    $zused=$Fld[1];
    $tracesm=0;$sigma=5;$bias=0;$bias2=0;
    @ids=split('_',$id);
    
    $mouchard="$id.mouchard1d";
    $lines="redshift.lines";
    @wl=@wlsky=();
    @flux=@fluxsky=();
    if(-e $mouchard)
    {
      open(MOUCHARD,$mouchard);
      ($txt)=split(' ',<MOUCHARD>);
#      ($txt2)=split(' ',<MOUCHARD>);
#      ($sky)=split(' ',<MOUCHARD>);
      ($wlmin,$wlmax)=split(' ',<MOUCHARD>);
      ($fluxmin,$fluxmax)=split(' ',<MOUCHARD>);
      ($lines)=split(' ',<MOUCHARD>);
      ($zused)=split(' ',<MOUCHARD>);
      ($tracesm,$sigma,$bias,$bias2)=split(' ',<MOUCHARD>);
      close(MOUCHARD);
      open(TXT,$txt);
      $i=0;
      while(<TXT>)
      {
        ($test1,$test2)=split;
        push(@wl,$test1); 
        push(@flux,$test2); 
        $i++;
      }
      $ni=$i;
      close(TXT);

#      open(TXT,$txt2);
#      $i=0;
#      while(<TXT>)
#      {
#        ($test1,$test2)=split;
#        push(@wl2,$test1);
#        push(@flux2,$test2);
#        $i++;
#      }
#      $ni2=$i;
#      close(TXT);
      
#      if(!(-e $sky)) {$sky="sky.sky";}

#      open(SKY,$sky);
#      $i=0;
#      while(<SKY>)
#      {
#        ($test1,$test2)=split;
#        push(@wlsky,$test1); 
#        push(@fluxsky,sqrt(abs($test2))); 
#        $i++;
#      }
#      $nsky=$i;
#      close(SKY);
    }
    else
    {
      $txt="./".$id2.".txt";
      $i=0;
      open(TXT,$txt)||die"Cannot find $txt";
      while(<TXT>)
      {
        ($test1,$test2)=split;
        push(@wl,$test1); 
        push(@flux,$test2); 
        if($i==0)
        {
          $fluxmin=$fluxmax=$test2;
          $wlmin=$wlmax=$test1;
        }
        else
        { 
          if($test2>$fluxmax) {$fluxmax=$test2;}
          if($test2<$fluxmin) {$fluxmin=$test2;}
          if($test1>$wlmax) {$wlmax=$test1;}
          if($test1<$wlmin) {$wlmin=$test1;}
        }
        $i++;
      }
      $ni=$i;
      close(TXT);

#      $sky="sky.sky";
#
#      open(SKY,$sky);
#      $i=0;
#      while(<SKY>)
#      {
#        ($test1,$test2)=split;
#        push(@wlsky,$test1); 
#        push(@fluxsky,sqrt(abs($test2))); 
#        $i++;
#      }
#      $nsky=$i;
#      close(SKY);

    }
    &readlines;
    if($sigma>0) {&calcsm;}

    $pgdevice = "/xserve";
    $pgdevice2 = $id."_1d.ps\/CPS";
    system("rm ".$id."_1d.ps");

    print "LIMITS=$wlmin $wlmax $fluxmin $fluxmax\n";

    $flag=0;
    while($flag==0)
    {
      pgopen($pgdevice);
      &trace;
      $dummy = <STDIN>;
      if($dummy eq "\n") {print("OK... Je passe au suivant !");$flag=1;}
      else
      {
         @Fld=split(' ',$dummy);
         if($Fld[0] eq "x") {$wlmin=$Fld[1];$wlmax=$Fld[2];}
         if($Fld[0] eq "y") {$fluxmin=$Fld[1];$fluxmax=$Fld[2];}
         if($Fld[0] eq "z") {$zused=$Fld[1];}
         if($Fld[0] eq "l") {if (!(-e "$id".".lines"))
                             {system("cp $lines $id".".lines");}
                             system("vi $id".".lines");
                             $lines=$id.".lines";&readlines;}

         
         if($Fld[0] eq "s") { $sigma=$Fld[1]; $bias=$Fld[2]; $bias2=$Fld[3];
                              if($sigma>0) {&calcsm; $tracesm=1;}
                            }
      }
      pgend;
    }

    pgopen($pgdevice2);
    &trace;
    pgend;
    
    open(MOUCHARD,">".$mouchard);
    print MOUCHARD "$txt\n";
#    print MOUCHARD "$txt2\n";
#    print MOUCHARD "$sky\n";
    print MOUCHARD "$wlmin $wlmax\n";
    print MOUCHARD "$fluxmin $fluxmax\n";
    print MOUCHARD "$lines\n";
    print MOUCHARD "$zused\n";
    print MOUCHARD "$tracesm $sigma $bias $bias2\n";
    close(MOUCHARD);
}
close(IN);


sub trace{
    pgsch(1.5);
    pgslw(3);
    pgsvp(0.10,0.99,0.15,0.89);
    pgswin($wlmin/(1+$zused),$wlmax/(1+$zused),$fluxmin,$fluxmax);
    pgbox("CMTS",0,0,"C",0,0);
    pgswin($wlmin,$wlmax,$fluxmin,$fluxmax);
    pgbox("BNTS",0,0,"BNTS",0,0);
    pgbox("C",0,0,"CTS",0,0);
    #pglabel("Wavelength (Ansgtroms)","Flux (ergs.s\\u-1\\d.cm\\u-2\\A\\u-1","$id z=$z"); # Labels
    pglabel("Observed Wavelength (\\A)","Flux ergs.s\\u-1\\d.cm\\u-2\\d\\A\\u-1","z=$z restframe Wavelength (\\A)"); # Labels
    
    pgsci(4);
    #pgtext($wlmin+0.02*($wlmax-$wlmin),$fluxmin+0.95*($fluxmax-$fluxmin),"z=$z");
    pgsci(2);
    #pgtext($wlmin+0.02*($wlmax-$wlmin),$fluxmin+0.85*($fluxmax-$fluxmin),"(z=$z2)");

    #shade bad regions
    pgsci(3);
    pgsfs(3);
    pgshs(45,0.5,0.0);
    #pgrect(5500,5585,$fluxmin,$fluxmax);
    #pgrect(5885,5895,$fluxmin,$fluxmax);
    pgrect(8425,8435,$fluxmin,$fluxmax);
    pgsfs(1);

    if($tracesm==1)
    {
      pgsci(2);
      pgline($ni,\@wl,\@smflux);
#      pgline($ni2,\@wl2,\@smflux2);
    }
      pgsci(1);
      pgline($ni,\@wl,\@flux);

    pgsls(4);
#    pgline($nsky,\@wlsky,\@fluxsky);
    
    $stepw=-($wlmax-$wlmin)*0.02;
    $stepf=($fluxmax-$fluxmin)*0.1;
    for($i=0;$i<$nlines;$i++)
    { 
      pgsci(4);
      pgslw(5);
      @x=@y=();
      push(@x,$wlines[$i]*(1+$zused));
      push(@x,$wlines[$i]*(1+$zused));
      push(@y,$fluxmin);
      push(@y,$fluxmax-1.*$stepf);
      pgline(2,\@x,\@y);
      @x=@y=();
      push(@x,$wlines[$i]*(1+$zused));
      push(@x,$wlines[$i]*(1+$zused));
      push(@y,$fluxmax-0.7*$stepf);
      push(@y,$fluxmax);
      pgline(2,\@x,\@y);
      if(($wlines[$i]*(1+$zused) > $wlmin) &&
        ($wlines[$i]*(1+$zused)<$wlmax)) 
      {
         pgtext($wlines[$i]*(1+$zused)+$stepw,$fluxmax-$stepf,$lbllines[$i]);
      }

#      pgsci(2);
#      pgslw(1);
#      @x=@y=();
#      push(@x,$wlines[$i]*(1+$z2));
#      push(@x,$wlines[$i]*(1+$z2));
#      push(@y,$fluxmin);
#      push(@y,$fluxmax-1.5*$stepf);
#      pgline(2,\@x,\@y);
#      @x=@y=();
#      push(@x,$wlines[$i]*(1+$z2));
#      push(@x,$wlines[$i]*(1+$z2));
#      push(@y,$fluxmax-1.2*$stepf);
#      push(@y,$fluxmax);
#      pgline(2,\@x,\@y);
#      if(($wlines[$i]*(1+$z2) > $wlmin) &&
#        ($wlines[$i]*(1+$z2)<$wlmax)) 
#      {
#         pgtext($wlines[$i]*(1+$z2)+$stepw,$fluxmax-1.5*$stepf,$lbllines[$i]);
#      }
    }
    pgsls(1);

   @skylinex1=(6290,6290,6310,6310,6290);
   @skyliney1=(fluxmin,fluxmax,fluxmax,fluxmin,fluxmin);
   pgsfs(3);
   pgpoly(5,\@skylinex1,\@skyliney1);
}

sub readlines
{
    print "Reading $line\n";
    open(LINES,$lines)||die;
    $nlines=0;
    @wlines=@lbllines=();
    while(<LINES>)
    {
      ($test1,$test2)=split;
      push(@wlines,$test1);
      push(@lbllines,$test2);
      $nlines++;
    }
    close(LINES);
}

sub calcsm
{
           #smooth spectrum here
           $box=5.0*$sigma;
           $box2=5.0*$sigma;
           for($i=0;$i<$ni;$i++)
           { 
              $j1 = int($i-$box);
              $j2 = int($i+$box);
              if($j1<0) {$j1=0;}
              if($j2<0) {$j2=0;}
              if($j1>$ni-1) {$j1=$ni-1;}
              if($j2>$ni-1) {$j2=$ni-1;}
     
              $smflux[$i]=0.0;
              $norm=0.0;
              for($j = $j1;$j<=$j2;$j++)
              {
                 $fac = exp(-0.5*((($j-$i)/$sigma)**2.0));
                 $smflux[$i] += $fac*$flux[$j];
                 $norm = $norm + $fac;
              }
              $smflux[$i]=$smflux[$i]/$norm + $bias;
           }
#           for($i=0;$i<$ni2;$i++)
#           {
#              $j1 = int($i-$box2);
#              $j2 = int($i+$box2);
#              if($j1<0) {$j1=0;}
#              if($j2<0) {$j2=0;}
#              if($j1>$ni2-1) {$j1=$ni2-1;}
#              if($j2>$ni2-1) {$j2=$ni2-1;}
#
#              $smflux2[$i]=0.0;
#              $norm=0.0;
#              for($j = $j1;$j<=$j2;$j++)
#              {
#                 $fac = exp(-0.5*((($j-$i)/$sigma)**2.0));
#                 $smflux2[$i] += $fac*$flux2[$j];
#                 $norm = $norm + $fac;
#              }
#              $smflux2[$i]=$smflux2[$i]/$norm + $bias2;
#           }
}

